Protograph LDPC Code Design for Asynchronous Random Access

This work addresses the physical layer channel code design for an uncoordinated, frame- and slot-asynchronous random access protocol. Starting from the observation that collisions between two users yield very specific interference patterns, we define a surrogate channel model and propose different protograph low-density parity-check code designs. The proposed codes are both tested in a setup where the physical layer is abstracted, as well as on a more realistic channel model, where finite-length physical layer simulations of the entire asynchronous random access scheme, including decoding are carried out. We find that the abstracted physical layer model overestimates the performance when short blocks are considered. Additionally, the optimized codes show gains in supported channel traffic - a measure of the number of terminals that can be concurrently accommodated on the channel - of around 17% at a packet loss rate of 10^{-2} w.r.t. off-the-shelf codes.

==> Tex/Dec_Region.tex <==
\section{Decoding Region}
For the code design, we made use of a simplified surrogate channel model. For the numerical results in Section~\ref{sec:results} we drop the surrogate model and simulate  more realistic \ac{RA} collision channels. The first set of numerical results makes the use of a physical layer abstraction where the interference is Gaussian, but not necessarily constant over the $\alpha \ns$ symbols. The physical layer is abstracted, since a  threshold based model is used to decide whether decoding is successful or not \cite{Pulini2013}. We then drop the assumption of Gaussian interferer and threshold based decoding and provide simulation results for the \ac{RA} scheme where the physical layer is implemented.

\subsection{Decoding Region for Gaussian Interference with Capacity Achieving Code}
\label{sec:decRegCA}
Opposed to the surrogate channel model in Section~\ref{sec:surrogate} we realistically assume that packets are received with varying level of interference. Thus, we resort to a \emph{block interference channel} \cite{McEliece1984,Clazzer18:ECRA}, where a packet experiences various blocks of constant interference.

Let us  call $m$ the maximum number of interferers affecting a reference packet. It is clear that up to $m+1$ different blocks might be present over the considered packet. The interference is assumed to be drawn from a complex white Gaussian process $\mathcal{CN}(0,2\inter)$, with $\inter$ being the interference variance per dimension (see also Section \ref{sec:gim}). Recall that the received signal power is normalized to $\frac{\sPw}{2}=\frac{1}{2}$, i.e., all interferers have the same power.  Define $\setI=\left\{\frac{1}{2}, 1, \frac{3}{2}, \ldots , \frac{m}{2}\right\} = \left\{\frac{j}{2} \mid  j=1,\ldots,m\right\}$ the interference set, clearly the interference variance  per dimension $\inter \in \setI$. We now associate to each element of $\mathcal{S}$ the corresponding fraction $\alpha_j$ of an interfered packet. Given the vectors $\BnPI=\left[\noise+\frac{1}{2}=\nPI_1,\ldots,\noise+\frac{m}{2}=\nPI_m\right]$ and $\bm{\alpha}=\left[\alpha_1,\ldots,\alpha_m\right]$, and recalling
$\Ca\left(\nPI\right)$ as the \ac{QPSK} constraint \ac{AWGN} channel capacity for a given $\nPI$, the outage capacity $\Capa$ for our surrogate channel model under the Gaussian interference assumption is
%
\begin{equation}
\label{eq:TSC_full}
\Capa(\bm{\alpha}, \noise, \BnPI) = \left(1-\sum_{j=1}^{m}\alpha_j\right) \,\Ca\left(\frac{1}{2\noise}\right) + \alpha_1 \, \Ca\left(\frac{1}{2\nPI_1}\right)+\dots+ \alpha_m \, \Ca\left(\frac{1}{2\nPI_m}\right).
\end{equation}
%
For a fixed transmission rate $\rate$, we define the decoding region $\rvDec$ \cite{Boutros2005,Pulini2013} as
\begin{align}\label{eq:dec_reg_full}
\rvDec &= \Bigg\{ \BnPI \in \mathbb{R}_{+}^{m}, \bm{\alpha} \in \left[0,1\right]^{m} \mid \sum_{j=1}^{m} \alpha_j \leq 1 \wedge \rate < \Capa(\BnPI, \noise, \bm{\alpha}) \Bigg\}
\end{align}
Every $m$-user collision resulting in $(\bm{\alpha}, \noise, \BnPI) \in \rvDec$ can be resolved. The impact of a non-capacity achieving code on the asynchronous \ac{RA} protocol performance is difficult to estimate due to the \ac{SIC} process. A first possibility is to numerically evaluate the performance of a code which achieves a fraction of the outage capacity $\capBO\,\Capa<\Capa$ (with, $\capBO<1$). The decoding region for such a error correcting code is
%
\begin{align}\label{eq:dec_reg_full_2}
\rvDec &= \Bigg\{ \BnPI \in \mathbb{R}_{+}^{m}, \bm{\alpha} \in \left[0,1\right]^{m} \mid \sum_{j=1}^{m} \alpha_j \leq 1 \wedge \rate < \capBO\,\Capa(\BnPI, \noise, \bm{\alpha}) \Bigg\}
\end{align}
% 
Properly setting the fraction $\capBO$ we can evaluate the \ac{MAC} performance of a code able to achieve, e.g. $95\%$ of the outage capacity.

\subsection{Decoding Region for Gaussian Interference with LDPC Code}
\label{sec:decReg}

For  \ac{LDPC} protograph ensembles the decoding region is computed by modify the decoding region in~\eqref{eq:dec_reg_full} as
%
\begin{align}
\label{eq:dec_cond_full_code}
\rvDec &= \Bigg\{\BnPI \in \mathbb{R}^{m}_{+}, \bm{\alpha} \in \left[0,1\right]^{m} \mid \sum_{k=1}^{m} \alpha_k \leq 1 \wedge \IAPP(j) \rightarrow 1\,\forall j\in\{0, \ldots, n_b-1\}\Bigg\}.
\end{align}
%
Note that for the threshold computation, at most $p_b-n_b$ different blocks can considered, corresponding to the different variable node types.

This first assumption is useful to compare with the performance achieved by the capacity achieving code undergoing the decoding region defined in Section \ref{sec:decRegCA}, and will be complemented 
